THEMIS: Time, Heterogeneity, and Energy Minded Scheduling for Fair Multi-Tenant Use in FPGAs

Using correct design metrics and understanding the limitations of the underlying technology is critical to developing effective scheduling algorithms. Unfortunately, existing scheduling techniques used \emph{incorrect} metrics and had \emph{unrealistic} assumptions for fair scheduling of multi-tenant FPGAs where each tenant is aimed to share approximately the same number of resources both spatially and temporally. This paper introduces an enhanced fair scheduling algorithm for multi-tenant FPGA use, addressing previous metric and assumption issues, with three specific improvements claimed First, our method ensures spatiotemporal fairness by considering both spatial and temporal aspects, addressing the limitation of prior work that assumed uniform task latency. Second, we incorporate energy considerations into fairness by adjusting scheduling intervals and accounting for energy overhead, thereby balancing energy efficiency with fairness. Third, we acknowledge overlooked aspects of FPGA multi-tenancy, including heterogeneous regions and the constraints on dynamically merging/splitting partially reconfigurable regions. We develop and evaluate our improved fair scheduling algorithm with these three enhancements. Inspired by the Greek goddess of law and personification of justice, we name our fair scheduling solution THEMIS: \underline{T}ime, \underline{H}eterogeneity, and \underline{E}nergy \underline{Mi}nded \underline{S}cheduling. We used the Xilinx Zedboard XC7Z020 to quantify our approach's savings. Compared to previous algorithms, our improved scheduling algorithm enhances fairness between 24.2--98.4\% and allows a trade-off between 55.3$\times$ in energy vs. 69.3$\times$ in fairness. The paper thus informs cloud providers about future scheduling optimizations for fairness with related challenges and opportunities.

==> 3.design_old.tex <==

\section{The Proposed Scheduling}
% \vspace{.-.5em}
\label{sec:design}

This study presents a scheduling technique for fair spatiotemporal tenant allocation in cloud FPGAs.
The proposed methodology consists of three main initiatives.
First, it considers both the area workload and computational time load of the tenants in the scheduling policy to improve fairness.
\Aysucomments{This is not an initiative, this is your result! **How** you achieve this is your initiative! The same thing applies to the third.}
Second, it reduces slots' idle times and increases resource utilization while preserving fairness.
Third, it reduces energy costs while maintaining fairness among tenants and provides flexibility with energy and fairness trade-offs.
% \Arsalancomment{In this part, we show our scheduling policy, which uses both area workload and computation time to attain fairness.}

% \setlength{\textfloatsep}{0.1cm}
% \setlength{\floatsep}{0.1cm}
\input{our_scheduling_alg.tex}

% \vspace{-.75em}
\subsection{Implementation of the Scheduling Algorithm}
% \vspace{-0.5em}
Algorithm~\ref{alg:1} shows the pseudo-code of our proposed scheduling.
The algorithm takes the following inputs: the total number of slots, the number of tenants, the order of tenants' allocation requests, and the interval length.
Interval is a point in time when the scheduler evaluates all tenants to make allocation decisions.
The algorithm has four stages: configuration, initialization, competition, and PR execution.
\Aysucomments{Is this really required or optional? This can be done generically for any algorithm.  Does STFS explain these details?$\rightarrow$}
In the configuration stage, the algorithm initially profiles all PR slots and gathers information about the available area provided by each slot.
The subsequent step in the configuration is to profile the tenants and attain their area ($A$) and computation time ($CT$) information.
The proposed algorithm later uses these collected workloads and slots' capacity profiles to calculate the desired target allocation as defined in subsection~\ref{subsec: new_metric}.
Since the configuration is a static operation, we do not present it in the pseudo-code of our proposed scheduling. 
Between steps 1 and 3 in the algorithm, our scheduling policy ensures that all tenants' average allocation is initialized with $0$.
% \Arsalancomment{The theoretical allocation that each tenant should receive is the average allocation. The purpose here is to provide feedback to our scheduling algorithm. Our scheduling algorithm then attempts to minimize the difference between the desired allocation and the current allocation over the course of its operation.}

Our scheduling algorithm runs unless the $Task$ queue\footnote{$Tasks$ queue is implemented with the last input first output (LIFO) method}is empty, indicating that the assigned tasks are finished.
At every interval, the scheduling algorithm fetches a set of tenant requests from the $Task$ queue and then performs the initialization routine.
In the initialization stage, the algorithm places tenants in the first smallest slot available that they can fit into.
If the tenant matches a slot, its average allocation is increased based on its workload area ($A$) and time ($CT$) product.
We call this product ($A \times CT$) an adjustment value ($AV$).
\Aysuomments{Is AV something you invent or already exist in STFS.  Since they use area, they must have a similar metric? Try to use their metric if applicable.}
Since the average allocation is the mean of tenant allocation, the $AV$'s contribution to the subsequent mean calculation reduces after each passing interval.
Therefore, the proposed scheduling algorithm revises the tenant's average allocation accordingly.
Each tenant has its own $AV$, stored in the \textit{$Ts$} data structure.
The initialization routine has two goals: (i) it assures that all PR slots are used at all times, even if there is only one tenant, and so eliminates the need for competing with others. (ii) it avoids conflict when the tenants have an equal average allocation and $AV$ in the competition stage.


After the first slot-tenant match, the algorithm enters the competition stage where the scheduling algorithm compares the allocated and unallocated tenants.
This competition has a simple rule: a prospective tenant ($T$) acquires the slot if the previously assigned tenant ($S.Tenant$) has a higher average allocation even after $S.Tenant$'s average allocation is reduced accordingly with its $AV$.
If the tenant $S.Tenant$ loses the competition, the algorithm first reduces its average allocation and then pushes back to the $Tasks$ queue.
As the prospective tenant $T$ wins the competition against $S.Tenant$, its average allocation is increased, and its corresponding slot's record is updated with the new tenant's configurations.

The competition stage ensures that the tenant with the lowest average allocation is given priority for allocation at each interval.
If the present available capacity is insufficient to meet the needs of the first-highest priority tenant, the slot is assigned to the second-highest priority tenant. As a result, our approach minimizes idle times in slots and improves resource utilization while maintaining fairness.



The next and final stage is to carry out the PR operation after deciding the respective slots for tenants.
% The scheduler will request a PR if and only if the new tenant of the relevant slot ($S$) differs from the one in the previous interval.
% If and only if the relevant slot's ($S$) new tenant differs from the one in the previous interval, the scheduler will request a PR.
The algorithm requires the PR if and only if the new tenant of a slot differs from the prior interval.
As a result, the number of PR operations is decreased, thereby improving performance and reducing energy consumption.





%The presented algorithm pursues fairness with low energy and resource efficiency by considering both area and timing requirements of tasks.





\begin{figure}[t]
\centering
	\hspace{-.5em}
	\includegraphics[width=0.5\textwidth]{figures/example.png}
	 \vspace{-2.0em}
	\caption{An example illustrating the slot allocation using the proposed algorithm. Three applications: AES, FFT, and SHA with area demands $6$, $9$, and $4$ are competing for allocation on two FPGA slots. Slot allocation is shown for eleven intervals.}
	\vspace{-1.5em}
	\label{fig: example}
\end{figure}
% \vspace{-1.5em}



\subsection{Fairness and Resource Utilization}
Figure~\ref{fig: example} presents an example of our scheduling policy.
There are three tenants represented with three rectangles: AES (orange), FFT (blue), and SHA (purple).
Each tenant (IP) has a specific workload and their area workload is the height of their rectangles, while the computational time load is the width of the rectangles.
In this example, AES, FFT, and SHA require $2$, $3$, and $1$ units of area, and $3$, $3$, and $4$ units of time, respectively.
Therefore, their adjustment values ($AV$) are $6$ ($2\times3$), $9$ ($3\times3$), and $4$ ($1\times4$) units.
Additionally, the FPGA has two available slots whose area capacities are equal to their heights, therefore Slot-$1$ has $2$ area units and Slot-$2$ has $3$ area units.
Time intervals are shown as $tn$ where '$n$' ranges from $0$ to $11$.
There is also a score table that displays the allocation values of tenants across the scheduling progress.
The table illustrates the fairness over allocation values rather than averaged allocation values to avoid the complication introduced by mean computation.
Before the first allocation, the scheduler initializes all tenants with the same allocation number, which is 0.


At the first time interval ($t0$), the scheduler proceeds with the given tenant order, hence, AES and FFT are allocated first.
Since their $AV$s are $6$ and $9$, their allocations result in a score of $6$ and $9$.
% It also means that the priorities of AES and FFT are decreased by $6$ and $9$, respectively,  to $-6$ and $-9$.
To improve area utilization, our algorithm assigns the smaller tenant to the smaller slot; in this example, AES is allocated to Slot-$1$, whereas FFT occupies Slot-$2$.
%If the first IP (AES) is assigned Slot-2 rather than Slot-1, the scheduler will be unable to allocate FFT due to FFT's area constraint.
\begin{figure*}[t]
\centering
\vspace{-1em}
	\includegraphics[width=\textwidth]{figures/all_in_one.png}
	\vspace{-2.7em}
	\caption{Average slot allocation of proposed work on three FPGA slots with allocation interval set as $36$. (a) This Work (b) STFS (c) DRR (d) RRR (PRR). Demand for each accelerator is as per data specified in Table~\ref{tab:Resource Usage}. Desired Average Allocation is calculated as $1.243$ per tenant. The proposed work accomplishes desired allocation (red-line) for all tenants, whereas, prior works deviate from desired allocation, compromising fairness.} 
 % \Aysucomments{what is the red dashed line? You need to include it to the legends on the top.  And if it is within Y-axis bounds, please also show the desired average allocation of STFS.}
 
	\label{fig:Perfromance-Evaluation}
	\vspace{-1.5em}
\end{figure*}
Until the $4th$ interval, SHA competes with AES and FFT but cannot win the competition since the scheduler adjusts the allocation values of these two tenants with their $AV$s and obtains the same allocation value as SHA.\\
\indent
To win the competition, SHA must have a lower allocation value (\textit{i.e.,} a lower score) than the adjusted allocations of the other two tenants.
In this situation, the adjusted values of these tenants (AES, FFT) are $0$, which is identical to the SHA value, until the $t3$.
At the 4$th$ interval ($t3$), SHA is first allocated to Slot-$1$ since it has the lowest allocation value and its score is increased by $4$.
Furthermore, because SHA's score is $4$ and still lower than the other two tenants even after its first allocation, it obtains Slot-$2$ as well.
If the decision interval is larger than $3$ time-unit (in this example it is set to $1$), AES and FFT will first start a new execution at $t3$ and then will be swapped with SHA at $t4$ without completing their work.
As a result, the execution between $t3$ and $t4$ would be wasted.
But unlike the prior work~\cite{STFS}, our algorithm can work with short intervals and minimizes resource wasting.\\
\indent
AES receives Slot-$2$ at the 8$th$ interval ($t7$)  because it has a lower allocation value and so a lower score than FFT and SHA.
AES is assigned to Slot-$2$ rather than Slot-$1$ because the scheduler always assigns the smaller tenant to the smaller slot.
Finally, AES first loses its slot to FFT at the $11th$ interval but then acquires Slot-$1$ by winning the competition against SHA at the $12th$ interval. 


% \begin{figure*}[t!]
% \centering
% \vspace{-1em}
% 	\includegraphics[width=\textwidth]{figures/all_in_one.png}
% 	\vspace{-2.7em}
% 	\caption{Average slot allocation of proposed work on three FPGA slots with allocation interval set as $36$. (a) This Work (b) STFS (c) DRR (d) RRR (PRR). Demand for each accelerator is as per data specified in Table~\ref{tab:Resource Usage}. Desired Average Allocation is calculated as $1.243$ per tenant.}
% 	\label{fig:Perfromance-Evaluation}
% 	\vspace{-1.5em}
% \end{figure*}

% \vspace{-.35em}

\subsection{Interval Length Effect on Energy and Fairness}
% \vspace{-0.25em}
Interval is a time period where the scheduler evaluates all tenants and performs the allocation decision.
Although the prior work performs its scheduling with a fixed and long interval~\cite{STFS}, the interval length has a significant effect on fairness~\cite{RR_interval,1966schedule}.
On the one hand, short intervals increase the scheduler's responsiveness and prompt the scheduler to meet the target fairness in a short period of time.
Short intervals, on the other hand, encourage the scheduler to perform more PR operations, consuming more energy.
Hence, the interval length is the key element in the energy and fairness trade-off. 
Figure~\ref{fig:eng-fairness} substantiates this claim.
The ability of the scheduler to be able to support dynamically varying interval lengths might come at the expense of the scheduler's performance overhead.
% However, one PR operation's computational time load is around 10,000$\times$ larger than the scheduler's one full allocation routine's execution time.
However, one PR process takes significantly longer than (about 10,000$\times$ in Xilinx's Zynq FPGAs) one tenant's execution.
Therefore, short interval overhead on the scheduler's performance is negligible.


% \Arsalancomment {
% \subsection{Slot Area Effect on Fairness}
%  FPGAs are comprised of heterogeneous  resources, making it highly improbable for two slots to possess identical resources. STFS postulated the incorrect notion that smaller slots can be combined on the fly to accommodate tenants with higher resource demands. In our study, we have assumed that slot sizes are large enough that any tenant may be assigned to any available slot. Although this approach may result in some slots being underutilized, we must adhere to the vendor's imposed limitations.}

%\Seetalcomments{The ability of the scheduler to be able to support dynamically varying interval lengths might come at the expense of the scheduler's performance overhead. In case that overhead is negligible, we might want to mention such details here.}

% \Aysucomments{Results should be described in the later section}
% \Emrecomments{I really like this structure but if you are sure, we can remove it from here.}
% Figure~\ref{fig:eng-fairness} illustrates our main point and shows our scheduler energy and fairness performances based on different interval lengths.
% The y-axis of the figure represents the unfairness, which is quantified with the absolute sum of the difference between the tenant's success rate and the target allocation.
% The x-axis depicts the energy consumption, which is computed by multiplying the PR's energy need with the number of PR completions in the overall scheduler progression time.
% The figure shows that shorter intervals can provide a fairer result, the long interval optimizes the energy  efficiency.


% \Aysucomments{You need to do this step by step and give out the numbers.  Describe in details.... In this example, AES, FFT, and SHA requires two, three, and one units of area, and three, three, and four units of time, respectively. Therefore, executing them once will reduce their priority by X, Y, and Z units.  In the beginning, they are all initialzied to X, Y, and Z, Then, at time t0 Xand Y must be executed, resulting in a score of X and Y.  Then at t3, these algorithms complete their first execution.  If the decision interval is less than this amount (in this example it is set to X), then at t3 they will be ...}
% Since all IPs have the same priority and the scheduler proceeds in IP order, the scheduler allocates the first AES and FFT into the slots at the first interval (T0).
% Then, their score is increased meaning that priorities are decreased by 6 and 9.
% Until the 4th interval, SHA competes with AES and FFT but cannot win the competition because the success rates of these two IPs are still not lower than SHA's after the $RVP$ reduction.
% SHA acquires both slots at the fourth interval since its first priority reduction is 4 and still higher than the other two IPs.
% At the seventh interval, SHA maintains its lead over FFT with a one-unit difference in priority, but AES obtains one slot.

% \Emrecomments{I completed the sections above this paragraph and you can check it out $\rightarrow$}I need to say that look our scheduling policy does not keep any slot idle because it can work with a short interval.
% For example, if the interval was 4 instead of 1 then between the fourth and the fifth intervals the slots would be idle because AES and FFT would start but SHA would get their slots before they complete their executions.
% Then, I need to say that look my slots are not identical but I am trying to fit the smallest IP into the smallest slot that the IP can fit into.
% At the first interval, AES didn't get the second slot and so FFT was able to find a space.

% \Arsalancomment{Our algorithm tries to minimize area wastage and idle time using two optimizations. First, it tries to find a slot with a minimal area that could host the tenant's workload. \textit{e.g. }In Fig.~\ref{fig: example} if AES is allocated Slot-1 then FFT would not be able to occupy Slot-2 in that interval since it wouldn't be able to fit. Second, before vacating slots preemptively it tries to find a future tenant with similar requirements to reduce idle time and minimize unnecessary PR operations.
% }

% Consider the following scenario, where the application order is predetermined. The algorithm is initialized with the following inputs; the total number of slots, applications to allocate, and the overall execution time. The maximum number of slots available is directly responsible for the number of concurrent applications (hence referred to as IP) that can be configured. Each IP has a specified time it needs to finish an operation, and our algorithm needs to be aware of this time in order to make smart scheduling decisions. This time is computed on the hardware once during the initialization stage. This is a key parameter in the time domain of our technique and is referred to as the \textit{IP profiling stage}. Keep in mind that each IP's resource requirements are known. A suitable interval time ensures that each application has a fair chance of execution. This time interval is then dynamically tuned during the extended execution to help in better slot allocation.\newline
% After that, each IP is given a slot to execute in, provided that there are still vacant slots available for it to occupy. The slot with the minimal resource that can satisfy the area need of the particular IP is selected in order to manage the spatial resource effectively. We also keep a priority counter with an initial value of zero for each IP. If an IP successfully occupies the slot in a given time interval, its priority for following intervals is reduced. On the other hand, an IP that was unable to schedule in the current interval is given priority for the subsequent interval. Every time interval, the counter values are carried forward. This guarantees that an IP that was unsuccessful in getting a space in the current period will be given priority in subsequent intervals. The IP may execute several jobs if a task is finished far earlier than the end of an interval. A job is allowed to finish and avoid preemption if it is unfinished at the end of an interval.\newline
% The IP with the highest priority is given first consideration for allocation in the period that follows. If the resource which is currently available cannot satisfy the demands of the first-highest IP, the second-highest IP is assigned that slot. This guarantees that each time interval has a minimum amount of idle time. The following information is also taken into account before a slot is evacuated: if the next IP contender will be able to finish its execution before that time interval is up. If not, IP that is already using the slot is not flushed and will continue to use it for the next interval, and its priority counter is adjusted for future executions, accordingly. This is done in an effort to lessen the number of needless PR operations, which consume excessive power.\newline
% Figure~\ref{fig:target_alloc} illustrates an example that is executed using the proposed work in which each application is striving for a slot. Time intervals are shown as $T_{n}$ where 'n' ranges from zero to eleven. At the start of the execution, each application is assigned identical priorities. AES, FFT, and SHA have latencies \{3, 3, 4\}  and area requirements of \{2, 3, 1\}, respectively. In the first interval, AES and FFT  occupy the slots and are permitted to finish their executions till interval T3. Since SHA's denied allocation in the intervals before T4, in T4 its priority is higher and it is therefore permitted to fill both slots. Slots are once more allocated to SHA and AES from T6 to T9. AES is able to conclude its execution well before the next scheduling decision is determined. Our algorithm then gives the slot to the next IP with a higher priority, FFT, in order to reduce idle time. Since FFT had previously been refused access, its priority counter had risen.







% % What are the advantages of our scheduling algorithm?
% This work presents a fair scheduling algorithm that iterates each time interval, to find optimum slot allocations for each application. For each application, the system specifies the target allocation and tries to minimize the difference between the intended target and the current target. Our proposed methodology is presented in algorithm~\ref{alg:pol_mult_alg}. 
% \subsection{The Implementation of the Scheduling Algorithm}
% % How does our scheduling algorithm work?
% Consider the following scenario, where the application order is predetermined. The algorithm is initialized with the following inputs; the total number of slots, applications to allocate, and the overall execution time. The maximum number of slots available is directly responsible for the number of concurrent applications (hence referred to as IP) that can be configured. Each IP has a specified time it needs to finish an operation, and our algorithm needs to be aware of this time in order to make smart scheduling decisions. This time is computed on the hardware once during the initialization stage. This is a key parameter in the time domain of our technique and is referred to as the \textit{IP profiling stage}. Keep in mind that each IP's resource requirements are known. A suitable interval time ensures that each application has a fair chance of execution. This time interval is then dynamically tuned during the extended execution to help in better slot allocation.\newline
% After that, each IP is given a slot to execute in, provided that there are still vacant slots available for it to occupy. The slot with the minimal resource that can satisfy the area need of the particular IP is selected in order to manage the spatial resource effectively. We also keep a priority counter with an initial value of zero for each IP. If an IP successfully occupies the slot in a given time interval, its priority for following intervals is reduced. On the other hand, an IP that was unable to schedule in the current interval is given priority for the subsequent interval. Every time interval, the counter values are carried forward. This guarantees that an IP that was unsuccessful in getting a space in the current period will be given priority in subsequent intervals. The IP may execute several jobs if a task is finished far earlier than the end of an interval. A job is allowed to finish and avoid preemption if it is unfinished at the end of an interval.\newline
% The IP with the highest priority is given first consideration for allocation in the period that follows. If the resource which is currently available cannot satisfy the demands of the first-highest IP, the second-highest IP is assigned that slot. This guarantees that each time interval has a minimum amount of idle time. The following information is also taken into account before a slot is evacuated: if the next IP contender will be able to finish its execution before that time interval is up. If not, IP that is already using the slot is not flushed and will continue to use it for the next interval, and its priority counter is adjusted for future executions, accordingly. This is done in an effort to lessen the number of needless PR operations, which consume excessive power.\newline
% Figure~\ref{fig:target_alloc} illustrates an example that is executed using the proposed work in which each application is striving for a slot. Time intervals are shown as $T_{n}$ where 'n' ranges from zero to eleven. At the start of the execution, each application is assigned identical priorities. AES, FFT, and SHA have latencies \{3, 3, 4\}  and area requirements of \{2, 3, 1\}, respectively. In the first interval, AES and FFT  occupy the slots and are permitted to finish their executions till interval T3. Since SHA's denied allocation in the intervals before T4, in T4 its priority is higher and it is therefore permitted to fill both slots. Slots are once more allocated to SHA and AES from T6 to T9. AES is able to conclude its execution well before the next scheduling decision is determined. Our algorithm then gives the slot to the next IP with a higher priority, FFT, in order to reduce idle time. Since FFT had previously been refused access, its priority counter had risen.
% \input{our_scheduling_alg.tex}

% \begin{figure}[t]
% 	\includegraphics[width=0.5\textwidth]{figures/example.png}
% 	\caption{An example illustrating the slot allocation using the proposed algorithm. Three applications; AES, FFT, and SHA with demands 6,9, and 4 are competing for allocation on two FPGA slots. Slot allocation is shown for eleven intervals.}
% 	\label{fig:target_alloc}
% \end{figure}

% \subsection{Energy and Fairness}
% How does the interval affect the scheduling performance?


==> Scheduling_Algorithm.tex <==
\begin{algorithm}[t!]
\small

\renewcommand{\algorithmicrequire}{{\textbf{Input}:}}
\renewcommand{\algorithmicensure}{{Output:}}
\begin{algorithmic}[1]
\Require{$Slots, \: Ts \rightarrow$ Slots and tenant data set}
\Require{$Tasks \rightarrow$  Queued tenants' orders} 
\Require{$interval\ \rightarrow$ Scheduler evaluation period}
% \vspace{0.25em}
% \tikzmark{right}
% % \vspace{0.5em}
% \State \textit{Slots} = \texttt{Profile\_Slots}(S_N)$
% \tikzmark{top}
% \State $Ts$ = \texttt{Profile\_Tenants}(IP_N)$

% \State TargetAlloc = \:\; \texttt{Set\_Target}($Slots$, $Ts$) \AddNote{\hspace{2.6em} Configuration}

% \tikzmark{bottom}
% % \vspace{0.5em}
\ForEach {$T \in \mathcal $Ts}
    % \State T.AvgAlloc$\:\; \leftarrow 0$
    \State $T$.AvgAlloc $= 0$
\EndFor

% \vspace{-0.5em}
\While{{not} $Tasks$.\texttt{Empty}}
    \State \textit{Ts}$\:\leftarrow Tasks$.\texttt{DeQueue}()
    % \vspace{-0.5em}
    \While{${\texttt{isEmpty}(}\textit{Slots}{)}$}
        \tikzmark{top2}
    
        \State $S   = {\texttt{SmallestSlot}}(Slots)$
        \tikzmark{right2}
                
        \State $T{.}AvgAlloc$ $  =  {\texttt{Inc}}(T.AV)$ 
\AddNote{\hspace{3.2em}  Initialization}
        \State $S{.}Tenant  = {\texttt{Update}}(T)$
            
    \EndWhile
\tikzmark{bottom2}
    \ForEach {$S \in \mathcal Slots$}
    \tikzmark{top3}
        \ForEach {$T \in \mathcal Ts$}
            \If{$\texttt{Swapping}(T, S.Tenant)$}\tikzmark{right3}
                \State $T_{tmp} =  \texttt{Get}(S.Tenant)$
                \State $S.T     =\texttt{Update}(T)$
                \State $T.AvgAlloc$ $ =\texttt{Dec}(T.AV)$
                
               
                \State $T_{tmp} = \texttt{Inc}(T_{tmp}.AV)$
                 \AddNote{\hspace{2.75em}  Competition}
                 \State $Tasks.$\texttt{EnQueue}$(T_{tmp})$
                \State \textit{Ts} $ = \texttt{Update}(T_{tmp})$
            \EndIf
        \EndFor
         
    \EndFor
    \tikzmark{bottom3}
    \ForEach {$S \in \mathcal $\textit{Slots}}
        \tikzmark{top4}
        \If{$\texttt{isPRneeded}(S)$}
        \tikzmark{right4}

            \State ${\texttt{PerformPR}}(S)$
                                 \AddNote{\hspace{3.0em}  PR Execution}

        \EndIf       
    \EndFor
    \tikzmark{bottom4}
    \vspace{0.25em}
    \State ${\texttt{Wait\_Next\_Interval}}(interval)$
    \vspace{0.25em}
\EndWhile

\caption{Pseudo Code of Proposed Scheduling\Aysucomments{Print a copy of STFS scheduling algorithm and put it next to your screen.  For each different line ask yourself do I need this or not? E.g., Why do you profile (e.g. line 1) and why this is not shown in STFS? Once this is done, then check if there is **ANY** different terms uses, etc. between your solution and STFS.}}
\label{alg:1}
\end{algorithmic}
\setlength{\textfloatsep}{0.4cm}
\setlength{\floatsep}{0.4cm}
\end{algorithm}
\vspace{-2.5em}

\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right)!(top.north)!($(right)-(0,1)$)$) --  ($(right)!(bottom.south)!($(right)-(0,1)$)$);
\end{tikzpicture}

\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right2)!(top2.north)!($(right2)-(0,1)$)$) --  ($(right2)!(bottom2.south)!($(right2)-(0,1)$)$);
\end{tikzpicture}


\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right3)!(top3.north)!($(right3)-(0,1)$)$) --  ($(right3)!(bottom3.south)!($(right3)-(0,1)$)$);
\end{tikzpicture}

\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right4)!(top4.north)!($(right4)-(0,1)$)$) --  ($(right4)!(bottom4.south)!($(right4)-(0,1)$)$);
\end{tikzpicture}


% \begin{algorithm}[t!]
% \small

% \renewcommand{\algorithmicrequire}{{Input:}}
% \renewcommand{\algorithmicensure}{{Output:}}
% \begin{algorithmic}[1]
% \Require{$S_N, IP_N \rightarrow$  Number of slots and tenants}
% \Require{$T\_E \rightarrow$  Total execution time} 
% \Require{$Tasks \rightarrow$  Queued tenants' orders} 
% \Require{interval$\ \rightarrow$ Scheduler evaluation period}
% \State Slots $\leftarrow Profile\_Slots(S_N)$
% \State IPs$\:\; \leftarrow Profile\_IPs(IP_N)$
% \State IPs$\:\; \leftarrow Initialize\_IPs(IP_N)$
% \State Slots$\:\; \leftarrow Initialize\_Slots(IP_N)$
% \While{time$\:\leq\:T\_E$}
%     \State IPs$\:\leftarrow DeQueue\_IPs(Tasks)$
%     \ForEach {$ip \in \mathcal $IPs}
%         \If{$empty\_slot(S_N)$ }
%             \If{$find\_smallest\_slot(ip)$}
%                 \State IPs$\: \leftarrow Decrease\_Priority(ip.PAV)$
%                 \State Slots$\: \leftarrow Update\_Slots($Slots$,ip)$
%             \EndIf
%         \EndIf
%     \EndFor
%     \ForEach {$s \in \mathcal $Slots}
%         \State T1$\: \leftarrow get\_current\_IP(s)$
%         \ForEach {$ip \in \mathcal $IPs}
%             \If{$swapping(ip.PAV,$T1$.PAV)$}
%                 \State IPs$\: \leftarrow Decrease\_Priority(ip.PAV)$
%                 \State Slots$\: \leftarrow Update\_Slots($Slots$,ip)$
%                 \State IPs$\: \leftarrow Increase\_Priority($T1$.PAV)$
%                 \State IPs$\:\leftarrow EnQueue\_IPs(Tasks,$T1$ )$
%                 \State T1$\: \leftarrow get\_current\_IP(s)$
%             \EndIf
%         \EndFor
%     \EndFor
%     \ForEach {$s \in \mathcal $Slots}
%         \If{$PR\_needed(s)$}
%             \State $Perform\_PR(s)$
%         \EndIf   
%     \EndFor
%     \State time+=$interval$
% \EndWhile

% \caption{Pseudo Code of Proposed Scheduling}
% \label{alg:1}
% \end{algorithmic}
% \setlength{\textfloatsep}{0.4cm}
% \setlength{\floatsep}{0.4cm}
% \end{algorithm}
% \vspace{-2.5em}





==> comparison_table.tex <==
\begin{table}
\large
\caption{Comparison with prior work}
\label{tab:comparison}
\centering
\begin{tabular}{|c|c|c|c|c|c|}\hline

\multirow{2}{*}{\textbf{Work}} & \multirow{2}{*}{\textbf{Multi-Tenancy}}& \multirow{2}{*}{\textbf{Energy}} &  \multirow{2}{*}{\textbf{SOD}} &  \multirow{2}{*}{\textbf{\% Util.}}  & \multirow{2}{*}{\textbf{Lacks}}\\
                   &\textbf{Support}  &                  &         &          &       \\ \hline                                   
\hline
This Work               & Spatiotemporal         & 0.34 mJ &  0.77   &   98.7 & -                              \\ \hline
STFS~\cite{STFS}        & Spatiotemporal         & 0.63 mJ &  0.89   &   85.4 & Latency Awareness   \\ \hline
DRR                     & Spatial          & 0.57 mJ &  1.54   &   10.9 & Latency/Temporal Awareness \\ \hline
RRR                     & Spatial         & 0.72 mJ &  1.74   &   34.2 & Latency/Temporal Awareness  \\ \hline
PRR                     & No          & 0.68 mJ &  1.42   &   24.4 & Latency/Temporal Awareness  \\ \hline
Blaze~\cite{Blaze}      & No         & -       &  -      &   -    & Latency/Spatial/Temporal Awareness           \\ \hline
AmorphOS~\cite{AmorphOS}& No         & -       &  -      &   -    & Latency/Temporal Awareness \\ \hline
Coyote~\cite{Coyote}    & Temporal         & -       &  -      &   -    & Latency/Spatial Awareness \\ \hline
Fahmy et al~\cite{Fahmy}& No         & -       &  -      &   -    & Latency/Spatial/Temporal Awareness \\ \hline

\end{tabular}
% \footnotetext{ LA = Latency Awareness, TA = Temporal Awareness, SA = Spatial Awareness}
\end{table}

==> tried.tex <==
\begin{algorithm}[t!]
\small

\renewcommand{\algorithmicrequire}{{\textbf{Input}:}}
\renewcommand{\algorithmicensure}{{Output:}}
\begin{algorithmic}[1]
\Require{$Slots \rightarrow$ FPGA Slots}
\Require{$n \rightarrow$ Number of tenants}
\Require{$D$[i]$ \rightarrow$  i$th$ tenant's demand, $i\in \mathcal [1,n)$}
\Require{$AV$[i]$ \rightarrow$  i$th$ tenant's $AV$
\Require{$interval \rightarrow$ Scheduler evaluation period}
\Require{$AvgAlloc$[i]$ \rightarrow$ i$th$ tenant's average allocation}

\For{$i$ \textbf{from} $0$ \textbf{to} $n$}
    \State $AvgAlloc$[i]= $0$
\EndFor

% \vspace{-0.5em}
\While{{True}}
    \State $D$ = \texttt{getTenantRqst}()
    \For{$i$ \textbf{from} $0$ \textbf{to} $n$}
         \If{${\texttt{isEmpty}(}\textit{Slots}{)}$}
            \State $Slots   = {\texttt{smallestSlot}}(D$[i]$)$
            \State j   = ${\texttt{whichTenant}}(D$[i]$)$
            \State $AvgAlloc$[j] += $AV$[j]
         \EndIf
    \EndFor
\tikzmark{bottom2}
    \ForEach {$S \in \mathcal Slots$}
    \tikzmark{top3}
        \For{$i$ \textbf{from} $0$ \textbf{to} $n$}
            \If{$\texttt{Swapping}(D$[i]$, S)$}\tikzmark{right3}
                \State $j =  \texttt{getTenant}(S)$
                \State $AvgAlloc$[j] -= $AV$[j]
                \State $Slots   = {\texttt{smallestSlot}}(D$[i]$)$
                \State j   = ${\texttt{whichTenant}}(D$[i]$)$
                \State $AvgAlloc$[j] += $AV$[j]
            \EndIf
        \EndFor         
    \EndFor
    \tikzmark{bottom3}
    \ForEach {$S \in \mathcal $\textit{Slots}}
        \tikzmark{top4}
        \If{$\texttt{isPRneeded}(S)$}
        \tikzmark{right4}

            \State ${\texttt{PerformPR}}(S)$
                                 \AddNote{\hspace{3.0em}  PR Execution}

        \EndIf       
    \EndFor
    \tikzmark{bottom4}
    \vspace{0.25em}
    \State ${\texttt{Wait\_Next\_Interval}}(interval)$
    \vspace{0.25em}
\EndWhile

\caption{Pseudo Code of Proposed Scheduling\Aysucomments{Print a copy of STFS scheduling algorithm and put it next to your screen.  For each different line ask yourself do I need this or not? E.g., Why do you profile (e.g. line 1) and why this is not shown in STFS? Once this is done, then check if there is **ANY** different terms uses, etc. between your solution and STFS.}}
\label{alg:1}
\end{algorithmic}
\setlength{\textfloatsep}{0.4cm}
\setlength{\floatsep}{0.4cm}
\end{algorithm}
\vspace{-2.5em}

\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right)!(top.north)!($(right)-(0,1)$)$) --  ($(right)!(bottom.south)!($(right)-(0,1)$)$);
\end{tikzpicture}

\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right2)!(top2.north)!($(right2)-(0,1)$)$) --  ($(right2)!(bottom2.south)!($(right2)-(0,1)$)$);
\end{tikzpicture}


\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right3)!(top3.north)!($(right3)-(0,1)$)$) --  ($(right3)!(bottom3.south)!($(right3)-(0,1)$)$);
\end{tikzpicture}

\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
 ($(right4)!(top4.north)!($(right4)-(0,1)$)$) --  ($(right4)!(bottom4.south)!($(right4)-(0,1)$)$);
\end{tikzpicture}


% \begin{algorithm}[t!]
% \small

% \renewcommand{\algorithmicrequire}{{Input:}}
% \renewcommand{\algorithmicensure}{{Output:}}
% \begin{algorithmic}[1]
% \Require{$S_N, IP_N \rightarrow$  Number of slots and tenants}
% \Require{$T\_E \rightarrow$  Total execution time} 
% \Require{$Tasks \rightarrow$  Queued tenants' orders} 
% \Require{interval$\ \rightarrow$ Scheduler evaluation period}
% \State Slots $\leftarrow Profile\_Slots(S_N)$
% \State IPs$\:\; \leftarrow Profile\_IPs(IP_N)$
% \State IPs$\:\; \leftarrow Initialize\_IPs(IP_N)$
% \State Slots$\:\; \leftarrow Initialize\_Slots(IP_N)$
% \While{time$\:\leq\:T\_E$}
%     \State IPs$\:\leftarrow DeQueue\_IPs(Tasks)$
%     \ForEach {$ip \in \mathcal $IPs}
%         \If{$empty\_slot(S_N)$ }
%             \If{$find\_smallest\_slot(ip)$}
%                 \State IPs$\: \leftarrow Decrease\_Priority(ip.PAV)$
%                 \State Slots$\: \leftarrow Update\_Slots($Slots$,ip)$
%             \EndIf
%         \EndIf
%     \EndFor
%     \ForEach {$s \in \mathcal $Slots}
%         \State T1$\: \leftarrow get\_current\_IP(s)$
%         \ForEach {$ip \in \mathcal $IPs}
%             \If{$swapping(ip.PAV,$T1$.PAV)$}
%                 \State IPs$\: \leftarrow Decrease\_Priority(ip.PAV)$
%                 \State Slots$\: \leftarrow Update\_Slots($Slots$,ip)$
%                 \State IPs$\: \leftarrow Increase\_Priority($T1$.PAV)$
%                 \State IPs$\:\leftarrow EnQueue\_IPs(Tasks,$T1$ )$
%                 \State T1$\: \leftarrow get\_current\_IP(s)$
%             \EndIf
%         \EndFor
%     \EndFor
%     \ForEach {$s \in \mathcal $Slots}
%         \If{$PR\_needed(s)$}
%             \State $Perform\_PR(s)$
%         \EndIf   
%     \EndFor
%     \State time+=$interval$
% \EndWhile

% \caption{Pseudo Code of Proposed Scheduling}
% \label{alg:1}
% \end{algorithmic}
% \setlength{\textfloatsep}{0.4cm}
% \setlength{\floatsep}{0.4cm}
% \end{algorithm}
% \vspace{-2.5em}




